A Benchmark for Low-Switching-Cost Reinforcement Learning

A ubiquitous requirement in many practical reinforcement learning (RL) applications, including medical treatment, recommendation system, education and robotics, is that the deployed policy that actually interacts with the environment cannot change frequently. Such an RL setting is called low-switching-cost RL, i.e., achieving the highest reward while reducing the number of policy switches during training. Despite the recent trend of theoretical studies aiming to design provably efficient RL algorithms with low switching costs, none of the existing approaches have been thoroughly evaluated in popular RL testbeds. In this paper, we systematically studied a wide collection of policy-switching approaches, including theoretically guided criteria, policy-difference-based methods, and non-adaptive baselines. Through extensive experiments on a medical treatment environment, the Atari games, and robotic control tasks, we present the first empirical benchmark for low-switching-cost RL and report novel findings on how to decrease the switching cost while maintain a similar sample efficiency to the case without the low-switching-cost constraint. We hope this benchmark could serve as a starting point for developing more practically effective low-switching-cost RL algorithms. We release our code and complete results in https://sites.google.com/view/low-switching-cost-rl.

==> 40dqn.tex <==
\yf{move 4.3 into sec 5}
%\yw{
	In this section, we develop a fully deterministic version of the state-of-the-art Q-learning algorithm, Rainbow DQN.
%} 
\xss{Describe the general framework of low-switching-cost RL}


%In this section, we will introduce how to implement a deterministic Rainbow DQN with a policy switching criterion.
% This implementation combines six DQN tricks and the policy is always deterministic.
%and can play many Atari games at human-level, then we introduce several strategies we adopt to reduce the switching times when training the Rainbow based DQN.

\subsection{Deterministic Q-network:}
%\yw{\textbf{}}
%\simon{@Shusheng: We don't need to mention 6 tricks here any more. Just add a description how to use deterministic rainbow.}
%\xss{
%We adopt Rainbow DQN to demonstrate our switching strategies. 
%\yw{
In its original form, Ranbow DQN adopts the Noisy Net \cite{Fortunato2018NoisyNF} technique to produce stochastic actions at training time for sufficient exploration. 
%}
%We first discuss how to make Rainbow DQN always output deterministic policies.
%Recall that to explore more efficiently, Rainbow adopts the Noisy Net \cite{Fortunato2018NoisyNF}, which makes the policy stochastic. 
To obtain a deterministic policy that explores, we remove Noisy Net 
%\yw{
while employing an exploration bonus during training.
% The aim is that with an adaptive policy deployment scheduling, the exploration bonus could encourage the Q-network visit diverse states.
%} 
%\yw{
	Specifically, when the deployed policy interacts with the environment, the action is chosen to maximize the Q-function, and after getting a transition $(x_t,a_t,r_{t+1},x_{t+1})$, we compute an additional exploration bonus $r^+(x_{t+1})$ to the original reward $r_{t+1}$.
%}

We employ the count-based exploration described in the previous section, 
%\yw{
	with exploration bonus 
%	$r^+$ 
%	by } %. When the deployed policy interacts with the environment, it selects the action which maximizes the $Q$-function. After obtaining the reward by taking this action, an exploration bonus 
$r^+(x) = \frac{\beta}{\sqrt{n(\phi(x))}}$. % is added into the reward.	 
%\yw{
Here $\phi(x)$ denotes a predefined feature function for state $x$, which is critical for high-dimensional state spaces such as images. Particularly, we consider a random projection function for image space in our paper as follows~\cite{Tang2017ExplorationAS}:
%}
%\xss{The hash function is described as follows:
%\xss{
\begin{enumerate}
 \item Initialize a fixed matrix $A$ with i.i.d entries from a standard Gaussian distribution $\mathcal{N}(0,1)$.
 \item $\phi(\cdot) = sgn(Ag(\cdot))$
\end{enumerate}
where $g$ is the flatten function.
%}
%}
% The original Rainbow contains six extensions, involving Double Q-learning, Prioritized Replay, Dueling Networks, Multi-step Learning, Distributional RL, and Noisy Nets. To make the policy deterministic but still keep exploring during training, we remove Noisy Net and adopt Count-Based exploration.


\subsection{DQN with a Policy Switching Criterion}
Rainbow updates the policies which interacts with the environment directly.
These policies usually switch millions of times during the training process (since the parameters are updated millions of times). 
In our implementation, we add an online policy in addition to the original deployed policy that interacts with the environment.
The deployed policy collects the data for the experience replay buffer, while the online policy is frequently updated when training. 
The deployed policy is replaced with the online policy the switching criterion is met, which we will discuss in more detail in the next section. The algorithm of deterministic switching Rainbow is shown in Algorithm \ref{alg:rainbow}.

%\simon{Define $H_{max}$, $H_{start}$, $H_{target}$ formally}
%\simon{@Shusheng: for notations, use $\mathrm{\cdot}$, for example, $\theta_{\mathrm{online}}$}
% \begin{algorithm*}[t]
% \caption{Deterministic Switching Rainbow}
% \label{alg:rainbow}
%     \begin{algorithmic}[1] 
%         \State{Initialize parameters $\theta_{\mathrm{online}}, \theta_{\mathrm{deployed}}, \theta_{\mathrm{target}}$ for online policy, deployed policy and target policy, initialize an empty replay buffer $D$. Denote the state encoder in online policy and deployed policy as $f_{\mathrm{online}}$ and $f_{\mathrm{deployed}}$}
%         % \State{Denote the state encoder in online policy and deployed policy as $f_{\mathrm{online}}$ and $f_{\mathrm{deployed}}$}
%         \State{Set the step to start training $H_{\mathrm{start}}$, the step to end training $H_{\mathrm{max}}$, $n(\mathrm{accumulated\_updates}) = 0,n(\mathrm{deployment})=0$} 
%         \State{Initialize state hash function $\phi({\cdot})$, $n_h(\phi(x_h), a_h) = 0$ for all $(x_h, a_h) \in \states\ \times \actions$ }
%         % \State{Set $n(\mathrm{accumulated\_updates}) = 0,n(\mathrm{deployment})=0$}
%         \For{h = 1 to $H_{\mathrm{max}}$}
%             \State{Select $a_h = \argmax_a Q_{\mathrm{deployed}}(x_h, a)$, execute action $a_h$  and observe reward $r_h$, state $x_{h+1}$ and $\mathrm{reset}$}
%             % \State{Execute action $a_h$  and observe reward $r_h$, state $x_{h+1}$ and $\mathrm{reset}$}
%             % \State{Compute the hash codes through for $x_h$, $\phi(x_h) = sgn(Ag(x_h))$}
%             % \LineComment{$A$ is a fixed matrix with i.i.d. entries drawn from a standard Gaussian distribution $\mathcal{N}(0, 1)$ and $g$ is a flat function}
%             % \State{Update the hash table counts, $n(\phi(x_h)) = n(\phi(x_h)) + 1$}
%             \State{Update the reward $r_h = r_h + \frac{\beta}{\sqrt{n(\phi(x_h))}}$}
%             % where $\phi$ is a hash function mapping the states into to lower dimensions.
%             \State{Store ($x_h$, $a_h$, $r_h$, $x_{h+1}$) in $D$, $n_h(\phi(x_h), a_h) = n_h(\phi(x_h), a_h) + 1$}
%             \If{$h > H_{\mathrm{start}}$}
%                 % \State{Sample a minibatch of transitions from $D$.}
%                 \State{Update $\theta_{\mathrm{online}}$ by stochastic gradient descent. Set $n(\mathrm{accumulated\_updates})$ = $n(\mathrm{accumulated\_updates})$ + 1}
%                 % \State{Set $n(\mathrm{accumulated\_updates})$ = $n(\mathrm{accumulated\_updates})$ + 1}
%                 % \If{$h \quad \% \quad H_{\mathrm{target}} == 0$ }
%                 %     \State{Update $\theta_{\mathrm{target}} = \theta_{\mathrm{online}}$}
%                 %     \State{Set $n(\mathrm{accumulated\_updates})$ = $n(\mathrm{accumulated\_updates})$ + 1}
%                 % \EndIf
%                 % \If{$\mathcal{J}(f_{\mathrm{deployed}}, f_{\mathrm{online}}, D, n(\mathrm{accumulated\_updates}),\mathrm{reset})) = true$}
%                 \If{$\mathcal{J}(\star) == \mathrm{true}$}
%                     \State{Update $\theta_{\mathrm{deployed}}$ = $\theta_{\mathrm{online}}, n(\mathrm{accumulated\_updates})=0, n(\mathrm{deployment}) = n(\mathrm{deployment}) + 1$}
%                     % \State{Update $n(\mathrm{accumulated\_updates})=0$}
%                     % \State{Update $n(\mathrm{deployment}) = n(\mathrm{deployment}) + 1$}
%                 \EndIf
%             \EndIf
%         \EndFor
%     \end{algorithmic}
% \end{algorithm*}

\subsection{RL with a Policy Switching Criterion}
Online RL algorithms updates the policy which interacts with the environment directly. These policies usually switch millions of times during the training process (since the parameters are updated millions if times). In our implementation, we add an online policy in addition to the original deployed policy that interacts with environment. The online policy is updated with RL algorithms but not interacts with the environment, while the deployed policy interacts with the environment and is unchanging until the switching criterion is met. The algorithm of low-switching-cost RL is shown in Algorithm~\ref{alg:low-switch-rl}. We will discuss policy switching criteria $\mathcal{J}$ in more detail in the next section.


\begin{algorithm*}[t]
\caption{Low-Switching-Cost RL}
\label{alg:low-switch-rl}
    \begin{algorithmic}[1] 
        \State{Initialize parameters $\theta_{\mathrm{online}}, \theta_{\mathrm{deployed}}$ for online policy and deployed policy , initialize an empty replay buffer $D$. $\mathrm{switching\ cost} = 0$} 
        % {Denote the state encoder in online policy and deployed policy as $f_{\mathrm{online}}$ and $f_{\mathrm{deployed}}$}
        % \State{Set $n(\mathrm{accumulated\_updates}) = 0,n(\mathrm{deployment})=0$} 
        % \State{Initialize state hash function $\phi({\cdot})$, $n_h(\phi(x_h), a_h) = 0$ for all $(x_h, a_h) \in \states\ \times \actions$ }
        % \State{Set $n(\mathrm{accumulated\_updates}) = 0,n(\mathrm{deployment})=0$}
        \For{h = 1 to $H_{\mathrm{max}}$}
            \State{Select $a_h$ by deployed policy, execute action $a_h$  and observe reward $r_h$, state $x_{h+1}$}
            \State{Store ($x_h$, $a_h$, $r_h$, $x_{h+1}$) in $D$}
            \State{Update $\theta_{\mathrm{online}}$ using $D$ and RL algorithm}
            \If{$\mathcal{J}(\star) == \mathrm{true}$}
                    \State{Update $\theta_{\mathrm{deployed}}$ = $\theta_{\mathrm{online}}$, $\mathrm{switching\ cost} = \mathrm{switching\ cost} + 1$}
            \EndIf
            
            % \If{$h > H_{\mathrm{start}}$}
            %     % \State{Sample a minibatch of transitions from $D$.}
            %     \State{Update $\theta_{\mathrm{online}}$ by stochastic gradient descent. Set $n(\mathrm{accumulated\_updates})$ = $n(\mathrm{accumulated\_updates})$ + 1}
            %     % \State{Set $n(\mathrm{accumulated\_updates})$ = $n(\mathrm{accumulated\_updates})$ + 1}
            %     % \If{$h \quad \% \quad H_{\mathrm{target}} == 0$ }
            %     %     \State{Update $\theta_{\mathrm{target}} = \theta_{\mathrm{online}}$}
            %     %     \State{Set $n(\mathrm{accumulated\_updates})$ = $n(\mathrm{accumulated\_updates})$ + 1}
            %     % \EndIf
            %     % \If{$\mathcal{J}(f_{\mathrm{deployed}}, f_{\mathrm{online}}, D, n(\mathrm{accumulated\_updates}),\mathrm{reset})) = true$}
            %     \If{$\mathcal{J}(\star) == \mathrm{true}$}
            %         \State{Update $\theta_{\mathrm{deployed}}$ = $\theta_{\mathrm{online}}, n(\mathrm{accumulated\_updates})=0, n(\mathrm{deployment}) = n(\mathrm{deployment}) + 1$}
            %         % \State{Update $n(\mathrm{accumulated\_updates})=0$}
            %         % \State{Update $n(\mathrm{deployment}) = n(\mathrm{deployment}) + 1$}
            %     \EndIf
            % \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm*}

==> 63suggestion.tex <==
\subsection{Best Practices}\label{sec:suggestion}
% \simon{I think only the last two points are "suggestions". The first two points are mainly showing the advantage of feature-based?}
%\yf{
We provide four suggestions on choosing an appropriate switching criterion from our experiments:
%	\\}

% \begin{wrapfigure}{l}{0.5\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/action_diff_feature_sim_v2.png}
%     \vspace{-1mm}
%     \caption{Action difference and feature similarity recorded on Pong. Higher feature similarity or lower action difference implies that the deployed policy and the online policy are closer.}
%     \label{fig:act_d_fea_s}
%     \vspace{-3mm}
% \end{wrapfigure}

% \begin{figure}
%     \centering
%     \begin{minipage}{0.45\textwidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/pong_episode_length.pdf}
%     \vspace{-1mm}
%     \caption{Episode length in Pong with feature-based criterion.}
%     \label{fig:pong_ep_length}
%     \end{minipage}
%     \begin{minipage}{0.45\textwidth}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/action_diff_feature_sim_v2.png}
%     \vspace{-1mm}
%     \caption{Action difference and feature similarity recorded on Pong. Higher feature similarity or lower action difference implies that the deployed policy and the online policy are closer.}
%     \label{fig:act_d_fea_s}
%     \end{minipage}
% \end{figure}

\paragraph{Try feature-based criterion instead of information-gain-based criteria for lower switching cost.} The theoretically guided criteria always suffer from larger switching cost or poorer sample efficiency compared with the feature-based criterion in practical benchmark tasks with modern RL algorithms. The proposed feature-based criterion is an initial step towards practical low-switching-cost RL. We believe more work is required to ultimately fill the gap between theory and practice. % The feature-based criterion exhibits much lower switching cost than theoretically guided criteria but also enjoys similar sample efficiency on all the benchmark environments.  

\paragraph{Try adaptive switching strategies instead of non-adaptive ones for better sample efficiency.} Although the non-adaptive switching criterion can achieve good performance if it knows an appropriate number of policy switches in advance, its performance is highly sensitive to the choice of the fixed switching interval (more in Appendix A). In contrast, adaptive criteria such as the feature-based criterion can automatically distribute the policy switches to different phases of training, which are easier to tune and often enjoy better sample efficiency. 
% \paragraph{Try fixed interval criterion as an initial attempt for low switching cost RL.} \yf{update after we get new results.} %\yf{
% The fixed interval criterion performs surprisingly well in Atari games, although its sample efficiency is slightly worse in some environments (see ``Road Runner''). We have also tried ``FIX\_100'' and ``FIX\_$10^4$'' and find that ``FIX\_$10^3$'' is the best for Atari games. Since the episode length of the tested games is also of magnitude $10^3$, it is likely that the best choice of fixed interval depends on the horizon of the environment.
% %}


\paragraph{Try feature-based instead of action-based criterion to better quantify policy differences.}
% \yf{
Empirically we observe that the switching cost of the action-based criterion is much higher than the feature-based criterion, indicating that actions often suffer from much larger noise than policy features. Fig.~\ref{fig:act_d_fea_s} shows that action difference changes drastically throughout the training process while feature similarity is much more stable. Even after the reward converges, we can still observe a significant action difference between the online policy and the deployed one. % , which indicates that action difference may not be an effective criterion. 
We suggest feature similarity as a more effective measure to quantify policy differences.
% In conclusion, feature similarity is more stable and credible to judge whether to switch.
%}

\paragraph{Switch only at reset time.}
We recommend switching the policy only when an episode resets.
The intuition is that switching policy too frequently in one episode may hinder exploration of the policies. Checking feature similarity only when an episode resets often help reduce the switching cost (see ablation studies in Appendix A). 
We also empirically find that the episode length in some tasks can go extremely large during training (see Fig.~\ref{fig:pong_ep_length}), which leads to a too staled deployed policy. So it can be necessary to force a policy switch when the deployed policy has been held steady for a long time. 
%}
% \begin{wrapfigure}{l}{0.5\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/action_diff_feature_sim_v2.png}
%     \vspace{-1mm}
%     \caption{Action difference and feature similarity recorded on Pong. Higher feature similarity or lower action difference implies that the deployed policy and the online policy are closer.}
%     \label{fig:act_d_fea_s}
%     \vspace{-3mm}
% \end{wrapfigure}
% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/pong_episode_length.pdf}
%     \vspace{-1mm}
%     \caption{Episode length in Pong with feature-based criterion.}
%     \label{fig:pong_ep_length}
%     \vspace{-3mm}
% \end{wrapfigure}


% \begin{wrapfigure}{l}{0.5\textwidth}
%     \centering
%     % \includegraphics[width=0.4\linewidth]{}
%     % \includegraphics[witdh=0.4\linewidth]{}
%     \subfigure{
%     \begin{minipage}[t]{1\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/action_diff_feature_sim_v2.png}
%     \caption{Action difference and feature similarity recorded on Pong. Higher feature similarity or lower action difference implies that the deployed policy and the online policy are closer.}
%     \label{fig:act_d_fea_s}
%     \end{minipage}
%     }
%     \subfigure{
%     \begin{minipage}[t]{1\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/pong_episode_length.pdf}
%     \caption{Episode length in Pong with feature-based criterion.}
%     \label{fig:pong_ep_length}
%     \end{minipage}
%     }
%     \label{fig:compare}
% \end{wrapfigure}
\iffalse
Secondly, we observe that  changing the policy with an adaptive interval may be better than a fixed interval. Focusing on the criteria $FIX\_10^4$ and $Adaptive\_10^2to10^4$, the adaptive criterion
switches the online policy fast at first and decrease its switching speed gradually, and in the end, the adaptive criterion would have the same speed as the fixed one.
Therefore, there is no significant difference between the total switching cost of these two criteria. However, we could observe that the adaptive criterion's performance is better than the fixed one when playing Beam Rider, Pong, Qbert, and they obtain similar performances in the rest games.

Lastly, we find our proposed feature-based criterion ($F\_0.98$) is the desired on that satisfy all four properties we discussed in Section~\ref{sec:intro}.
It significantly reduces the switching cost compared to ``None", and is smaller than $FIX\_10^2$.
While it incurs higher switching cost than $FIX\_10^3$, $FIX\_10^4$, and $Adaptive\_10^2to10^4$, \emph{on all environments} feature-based criterion consistently perform as well as ``None" in the sense that 1) it finds the optimal policy eventually, 2) it has the same sample efficiency as ``None".
On the other hand, other criteria sometime have significantly worse performance compared to ``None", so none of them is a generic solution.
\fi

%We believe such generality comes from that 
%n others. When maintaining the performances when playing all of these six games, this strategy could adjust the switching speeds depending on different environments and situations. We observe that when playing Battle Zone and Pong, where $FIX\_10^2$ outperforms $F\_10^3$ obviously, the feature-based strategy tries to increase the switching times and keep a similar performance with $FIX\_10^2$. In other games where there is no apparent difference between $FIX\_10^2$ and $FIX\_10^3$, the feature-based strategy keeps a comparable performance with the switching times between $FIX\_10^2$ and $FIX\_10^3$. So in the trade-off of performance and switching times, it is better to choose the feature-based strategy.


